Les conjectures de Weil : origines, approches, g\'en\'eralisations

Je retracerai l'histoire des conjectures de Weil sur le nombre de solutions d'\'equations polynomiales dans un corps fini et quelques unes des approches qui ont \'et\'e propos\'ees pour les r\'esoudre. The Weil conjectures: origins, approaches, generalizations. I recount the history of the conjectures by Weil on the number of solutions of polynomial equations in finite fields, and some of the approaches that have been proposed to solve them.

==> frenchbst.tex <==
 % This is babelbst.tex for English.
 % It should serve as a model for other languages.
 % Alternatively, store it under a different name (e.g. englbst.tex)
 % and then \input it with a command in babelbst.tex.
\def\bbland{et}                \def\bbletal{et~al.}
\def\bbleditors{\'editeurs}        \def\bbleds{\'eds.}
\def\bbleditor{\'editeur}          \def\bbled{\'ed.}
\def\bbledby{\'edit\'e by}
\def\bbledition{\'edition}        \def\bbledn{\'ed.}
\def\bblvolume{volume}          \def\bblvol{vol.}
\def\bblof{de}
\def\bblnumber{num\'ero}          \def\bblno{n\textsuperscript o}
\def\bblin{in}
\def\bblpages{pages}            \def\bblpp{p.}
\def\bblpage{page}              \def\bblp{p.}
\def\bbleidpp{pages}
\def\bblchapter{chapitre}        \def\bblchap{chap.}
\def\bbltechreport{Pr\'epublication}
\def\bbltechrep{Pr\'ep.}
\def\bblmthesis{M\'emoire de DEA}
\def\bblphdthesis{Th\`ese de doctorat}
\def\bblfirst{Premi\`ere}            \def\bblfirsto{1\textsuperscript{re}}
\def\bblsecond{Deuxi\`eme}          \def\bblsecondo{2\textsuperscript{e}}
\def\bblthird{Troisi\`eme}            \def\bblthirdo{3\textsuperscript{e}}
\def\bblfourth{Fourth}          \def\bblfourtho{4\textsuperscript{e}}
\def\bblfifth{Fifth}            \def\bblfiftho{5\textsuperscript{e}}
\def\bblst{\textsuperscript{re}}
  \def\bblnd{\textsuperscript{e}}  \def\bblrd{\textsuperscript{e}}
\def\bblth{\textsperscript{e}}
\def\bbljan{Janvier}  \def\bblfeb{F\'evrier}  \def\bblmar{Mars}
\def\bblapr{Avril}    \def\bblmay{Mai}       \def\bbljun{Juin}
\def\bbljul{Juillet}     \def\bblaug{Ao\^ut}    \def\bblsep{Septembre}
\def\bbloct{Octobre}  \def\bblnov{Novembre}  \def\bbldec{Decembre}


